Ultrafast carrier relaxation and its Pauli drag in photo-enhanced melting of solids

Ultrafast light-matter interaction is a powerful tool for the study of solids. Upon laser excitation, carrier multiplication and lattice acceleration beyond thermal velocity can occur, as a result of far-from-equilibrium carrier relaxation. The roles of electron-electron and electron-phonon scatterings are identified by first-principles dynamic simulations, from which a unified phase diagram emerges. It not only explains the experimentally-observed "inertial" melting but also predicts abnormal damping by Pauli Exclusion Principle with a new perspective on ultrahigh-intensity laser applications.

==> arXiv_1st (8th)/SM.tex <==
%\documentclass[aps, prl,preprint, groupedaddress, floatfix, superscriptaddress, showpacs]{revtex4-1} %showpacs preprint, reprint, twocolumn,longbibliography longbibliography,
%\usepackage[colorlinks,allcolors=blue]{hyperref}
%\usepackage{graphicx}
%\usepackage{epstopdf}
%\usepackage{dcolumn}
%\usepackage{bm}
%\usepackage{braket}
%
%\newcommand\fitwidth{1.0\linewidth}
%\newcommand\fullwidth{0.9\textwidth}
%
%\newcommand{\beginsupplement}{%
%	\setcounter{table}{0}
%	\renewcommand{\thetable}{S\arabic{table}}%
%	\setcounter{figure}{0}
%	\renewcommand{\thefigure}{S\arabic{figure}}%
%	\setcounter{equation}{0}
%	\renewcommand{\theequation}{S\arabic{equation}}%
%}

%\newcommand{\MyAbs}{using our recent developed time-dependent density function (TDDFT) method, we systematically studied the ultrafast dynamics of crystalline silicon under various conditions. Through analyzing the dynamics of phonons (ph), electrons (el) and photons together with their interplay, we emphasize that the carrier relaxation is a major factor for the full understanding of ultrafast structural changes. The hot electrons generated by the laser pulse are redistributed in energy through el-el and el-ph scattering. The thermalization accompanies and accelerates structural phase transition. Based on the diverse efficiencies of carrier relaxation under different temperatures and laser intensities, we picture the phase diagram of different melting dynamics. Not only the experimental observed inertial melting is reproduced at specific laser intensity and temperature range, but also an abnormal hindering of melting is predicted under the higher intensity. We demonstrated that the PA model fails to explain these dynamics due to the `rigid' PES assumption. It indicates that the phonon, electron and photon system should be treated at the same root to accurately describe the ultrafast structural changes.} %We proposed that the inertial dynamics is combined consequence of weakened bonds by excited electrons and thermal acceleration by el-ph scattering, as shown in Fig.~\ref{fig:inertialModel}(b). 

%\begin{document}
\beginsupplement
\section{Supplementary Materials}

\subsection{Carrier Scattering in TDDFT}
    	
We evaluate the state-to-state transition probabilities between TDKS orbitals during time evolution:
\begin{equation}
\label{projection}
P_{nn'\mathbf{k}} = \left|C_{nn'\mathbf{k}} \right|^2 = \left|\braket{v_{n\mathbf{k}}|S_k|u_{n'\mathbf{k}}}\right|^2,
\end{equation}
where $S_\mathbf{k}$ is the overlap matrix,  $u_{n'\mathbf{k}}$ is the time dependent Kohn-Sham (TDKS) orbitals and $\ket{v_{n\mathbf{k}}}$ is the adiabatic basis satisfying
\begin{equation}
\label{adiabaticBasis}
H_\mathbf{k}\ket{v_{n\mathbf{k}}(\mathbf{r})} = E_{n\mathbf{k}} S_\mathbf{k}\ket{v_{n\mathbf{k}}(\mathbf{r})}.
\end{equation}
where $H_\mathbf{k}$ is the Hamiltonian.
The population $\mathcal{q}_{n\mathbf{k}}$ of the adiabatic state $n\mathbf{k}$ is thus projected from the TDKS orbitals at a given time as:
\begin{equation}
\label{eq:excitation}
\mathcal{q}_{n\mathbf{k}} =  \sum_{n'\in n_{\mathbf{k},occ}} q_{n'\mathbf{k}} P_{nn'\mathbf{k}},
\end{equation}
where $n_{\mathbf{k},occ}$ is the occupied state at $\mathbf{k}$ point.
The number of excited electrons $n(t)$ is calculated as,
\begin{equation}
\label{eq:ExcitedElectrons}
n(t) = \sum_{unocc} \mathcal{q}_{n\mathbf{k}}(t),
\end{equation}

%\subsection{Describe the Scattering in TDDFT}
The scattering of carriers are described by the changes of $\mathcal{q}_{n\mathbf{k}}$ as a function of time. The increase of $\mathcal{q}_{n\mathbf{k}}$ occurs together with the decrease of $\mathcal{q}_{m\mathbf{k}}$, which represents the transition from adiabatic state $m$ to $n$. The transition is confined within the same $\mathbf{k}$, since $H_\mathbf{k}$ is independent subspace for each $\mathbf{k}$. Thus, only intra-$\mathbf{k}$ scattering is allowed in the simulation. This limitation requires a supercell to accurately describe the scattering process. With a infinite large supercell, all inter-$\mathbf{k}$ scatterings in unit cell are converted to intra-$\mathbf{k}$ scatterings, due to the band folding. 

%The density of states is a qualitative evaluation of the accuracy. The 



%\newpage
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{RMSDContour}
    \caption{(a) RMSD and (b) temperature contour maps as a function of time. }
    \label{fig:RMSDContour}
\end{figure}

%\newpage
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{cohp}
    \caption{Density of states (DOS) and crystal orbital Hamilton population (COHP) as a function of energy. The negative regime of COHP denotes bonding state, while the positive regime denotes the anti-bonding state.}
    \label{fig:cohp}   
\end{figure}

%\end{document}
